Transfer Learning for Segmentation Problems: Choose the Right Encoder and Skip the Decoder

It is common practice to reuse models initially trained on different data to increase downstream task performance. Especially in the computer vision domain, ImageNet-pretrained weights have been successfully used for various tasks. In this work, we investigate the impact of transfer learning for segmentation problems, being pixel-wise classification problems that can be tackled with encoder-decoder architectures. We find that transfer learning the decoder does not help downstream segmentation tasks, while transfer learning the encoder is truly beneficial. We demonstrate that pretrained weights for a decoder may yield faster convergence, but they do not improve the overall model performance as one can obtain equivalent results with randomly initialized decoders. However, we show that it is more effective to reuse encoder weights trained on a segmentation or reconstruction task than reusing encoder weights trained on classification tasks. This finding implicates that using ImageNet-pretrained encoders for downstream segmentation problems is suboptimal. We also propose a contrastive self-supervised approach with multiple self-reconstruction tasks, which provides encoders that are suitable for transfer learning in segmentation problems in the absence of segmentation labels.

==> figures/aeroplane/unet-old.tex <==
% This file was created by tikzplotlib v0.9.9.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}

\begin{axis}[
height=5cm,
legend cell align={left},
legend style={
  fill opacity=1,
  draw opacity=1,
  text opacity=1,
  at={(0.97,0.03)},
  anchor=south east,
  draw=white!80!black
},
tick align=outside,
tick pos=left,
width=7cm,
x grid style={white!69.0196078431373!black},
xlabel={Epoch},
xmajorgrids,
xmin=-5.5, xmax=313.5,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Dice Score},
ymajorgrids,
ymin=0.486526273190975, ymax=0.694396682083607,
ytick style={color=black}
]
\addplot [semithick, color0, mark=x, mark size=3, mark options={solid}]
table {%
9 0.599280476570129
19 0.621403336524963
29 0.634008526802063
39 0.645681619644165
49 0.652037501335144
59 0.658196449279785
69 0.658601820468903
79 0.660503268241882
89 0.665309131145477
99 0.666067183017731
109 0.664761304855347
119 0.670406639575958
129 0.673900663852692
139 0.676863431930542
149 0.677049040794373
159 0.674886167049408
169 0.676200747489929
179 0.675016105175018
189 0.679364681243896
199 0.677058041095734
209 0.678172707557678
219 0.681260645389557
229 0.678895771503448
239 0.675745487213135
249 0.679350197315216
259 0.676622450351715
269 0.677698731422424
279 0.672918021678925
289 0.678829848766327
299 0.674869477748871
};
\addlegendentry{pretrained}
\addplot [semithick, color1, mark=x, mark size=3, mark options={solid}]
table {%
9 0.512764692306519
19 0.540909945964813
29 0.572147369384766
39 0.575510144233704
49 0.593113720417023
59 0.589972853660583
69 0.628599643707275
79 0.638789534568787
89 0.6433265209198
99 0.643421053886414
109 0.635805010795593
119 0.652856647968292
129 0.656596958637238
139 0.656414449214935
149 0.659572720527649
159 0.665201783180237
169 0.658829569816589
179 0.660347819328308
189 0.670821130275726
199 0.665897190570831
209 0.663681507110596
219 0.671122431755066
229 0.668150663375854
239 0.669520676136017
249 0.666325151920319
259 0.672549486160278
269 0.666852355003357
279 0.684948027133942
289 0.674460291862488
299 0.671516239643097
};
\addlegendentry{random-decoder}
\addplot [semithick, color2, mark=x, mark size=3, mark options={solid}]
table {%
9 0.49597492814064
19 0.533290505409241
29 0.550220370292664
39 0.560526490211487
49 0.578805267810822
59 0.583416223526001
69 0.599714338779449
79 0.605206906795502
89 0.615546941757202
99 0.602414131164551
109 0.602348685264587
119 0.625627040863037
129 0.623918056488037
139 0.626441836357117
149 0.627706050872803
159 0.611042082309723
169 0.635018587112427
179 0.630387425422668
189 0.634584784507751
199 0.638905882835388
209 0.63821542263031
219 0.631551027297974
229 0.638888657093048
239 0.625717878341675
249 0.640228867530823
259 0.638881385326385
269 0.635106205940247
279 0.641626477241516
289 0.639375448226929
299 0.644034445285797
};
\addlegendentry{random}
\end{axis}

\end{tikzpicture}

==> figures/bus/resnet-old.tex <==
% This file was created by tikzplotlib v0.9.9.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}

\begin{axis}[
height=5cm,
legend cell align={left},
legend style={
  fill opacity=1,
  draw opacity=1,
  text opacity=1,
  at={(0.97,0.03)},
  anchor=south east,
  draw=white!80!black
},
tick align=outside,
tick pos=left,
width=7cm,
x grid style={white!69.0196078431373!black},
xlabel={Epoch},
xmajorgrids,
xmin=-3, xmax=261,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Dice Score},
ymajorgrids,
ymin=0.504619297385216, ymax=0.779912832379341,
ytick style={color=black}
]
\addplot [semithick, color0, mark=x, mark size=3, mark options={solid}]
table {%
9 0.638917565345764
19 0.659426867961884
29 0.677962124347687
39 0.661914110183716
49 0.703266859054565
59 0.717925786972046
69 0.714682698249817
79 0.719750165939331
89 0.721604406833649
99 0.731106758117676
109 0.725298702716827
119 0.740818083286285
129 0.745682060718536
139 0.732909142971039
149 0.760545015335083
159 0.767399489879608
169 0.737093091011047
179 0.753349721431732
189 0.756614446640015
199 0.75905567407608
209 0.744045972824097
219 0.744714319705963
229 0.759585678577423
239 0.760543584823608
249 0.745747745037079
};
\addlegendentry{pretrained}
\addplot [semithick, color1, mark=x, mark size=3, mark options={solid}]
table {%
9 0.517132639884949
19 0.562295198440552
29 0.581216752529144
39 0.612709999084473
49 0.599183797836304
59 0.632885694503784
69 0.619408249855042
79 0.661513328552246
89 0.647784948348999
99 0.667159020900726
109 0.668367266654968
119 0.665008246898651
129 0.677499771118164
139 0.676923751831055
149 0.682903409004211
159 0.678799867630005
169 0.674173533916473
179 0.693067669868469
189 0.695140659809113
199 0.640456140041351
209 0.69853949546814
219 0.6978600025177
229 0.686193704605103
239 0.709186136722565
249 0.700128436088562
};
\addlegendentry{random}
\addplot [semithick, color2, mark=x, mark size=3, mark options={solid}]
table {%
9 0.548849284648895
19 0.564988911151886
29 0.574775516986847
39 0.609650135040283
49 0.621670186519623
59 0.632321178913116
69 0.655023574829102
79 0.665805339813232
89 0.673016786575317
99 0.689751505851746
109 0.687379121780396
119 0.701191663742065
129 0.702453672885895
139 0.736357569694519
149 0.736788392066956
159 0.726502656936646
169 0.722129702568054
179 0.747486352920532
189 0.734455704689026
199 0.747444748878479
209 0.747248530387878
219 0.747504234313965
229 0.750778913497925
239 0.761645674705505
249 0.756188631057739
};
\addlegendentry{random-decoder}
\end{axis}

\end{tikzpicture}

==> figures/bus/resnet.tex <==
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
height=6cm,
legend cell align={left},
legend columns=2,
legend style={
  fill opacity=1,
  draw opacity=1,
  text opacity=1,
  at={(0.5,1.3)},
  anchor=north,
  draw=white!80!black,
  style={column sep=0.2cm}
},
tick align=outside,
tick pos=left,
width=7cm,
x grid style={white!69.0196078431373!black},
xlabel={Epoch},
xmajorgrids,
xmin=-0.5, xmax=208.5,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Dice Coef},
ymajorgrids,
ymin=0.479376070201397, ymax=0.840657688677311,
ytick style={color=black}
]
\addplot [semithick, color0, mark=x, mark size=3, mark options={solid}]
table {%
9 0.749181032180786
19 0.768976330757141
29 0.784484624862671
39 0.782566547393799
49 0.80383026599884
59 0.799732506275177
69 0.774044334888458
79 0.807013154029846
89 0.794789612293243
99 0.81143456697464
109 0.79976212978363
119 0.804109156131744
129 0.806172490119934
139 0.806680917739868
149 0.801862418651581
159 0.817336320877075
169 0.800456285476685
179 0.795554220676422
189 0.822798669338226
199 0.823730051517487
};
\addlegendentry{Segmentation}
\addplot [semithick, color1, mark=x, mark size=3, mark options={solid}]
table {%
9 0.511695384979248
19 0.545530736446381
29 0.579239189624786
39 0.617569208145142
49 0.650890827178955
59 0.665432929992676
69 0.710200548171997
79 0.730445086956024
89 0.755815982818604
99 0.776825368404388
109 0.78628808259964
119 0.7997887134552
129 0.790172696113586
139 0.803721129894257
149 0.817978501319885
159 0.813104033470154
169 0.821680963039398
179 0.824235796928406
189 0.820161938667297
199 0.824146747589111
};
\addlegendentry{Seg RD}
\addplot [semithick, color2, mark=x, mark size=3, mark options={solid}]
table {%
9 0.600777566432953
19 0.649967968463898
29 0.691806674003601
39 0.721601665019989
49 0.708280563354492
59 0.734398782253265
69 0.726153492927551
79 0.73738044500351
89 0.753463923931122
99 0.75335967540741
109 0.742675244808197
119 0.761210858821869
129 0.736369848251343
139 0.76499605178833
149 0.763383626937866
159 0.773019433021545
169 0.772840321063995
179 0.759884119033813
189 0.760068356990814
199 0.772546947002411
};
\addlegendentry{Classification}
\addplot [semithick, color3, mark=x, mark size=3, mark options={solid}]
table {%
9 0.495797961950302
19 0.512373745441437
29 0.589140892028809
39 0.581689596176147
49 0.654430687427521
59 0.635592639446259
69 0.625602602958679
79 0.642401397228241
89 0.657377481460571
99 0.674047231674194
109 0.678488612174988
119 0.692816972732544
129 0.693399786949158
139 0.670734405517578
149 0.700179278850555
159 0.705633878707886
169 0.700630903244019
179 0.691985130310059
189 0.698435664176941
199 0.700295686721802
};
\addlegendentry{Random}
\end{axis}

\end{tikzpicture}


==> figures/cars-pretrain/pretrain.tex <==
% This file was created by tikzplotlib v0.9.9.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}

\begin{axis}[
height=5cm,
legend cell align={left},
legend style={
  fill opacity=1,
  draw opacity=1,
  text opacity=1,
  at={(0.97,0.03)},
  anchor=south east,
  draw=white!80!black
},
tick align=outside,
tick pos=left,
width=7cm,
x grid style={white!69.0196078431373!black},
xlabel={Epoch},
xmajorgrids,
xmin=-4.45, xmax=93.45,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Dice Coef},
ymajorgrids,
ymin=0.452942961454392, ymax=0.999615794420242,
ytick style={color=black}
]
\addplot [semithick, color0, mark=x, mark size=3, mark options={solid}]
table {%
0 0.477791726589203
1 0.649876117706299
2 0.729708433151245
3 0.774443089962006
4 0.807051360607147
5 0.821054100990295
6 0.847062706947327
7 0.861398100852966
8 0.870990693569183
9 0.880178809165955
10 0.887636959552765
11 0.900332391262054
12 0.898422420024872
13 0.9036003947258
14 0.908873856067657
15 0.907822549343109
16 0.917531967163086
17 0.919430732727051
18 0.923601865768433
19 0.924760580062866
20 0.926386296749115
21 0.926817774772644
22 0.92965179681778
23 0.933721542358398
24 0.939481019973755
25 0.941910028457642
26 0.941825807094574
27 0.943332970142365
28 0.93622761964798
29 0.937844216823578
30 0.942298173904419
31 0.947042226791382
32 0.949973702430725
33 0.949531733989716
34 0.950142979621887
35 0.950774431228638
36 0.952368319034576
37 0.950814545154572
38 0.942693889141083
39 0.95141464471817
40 0.955217599868774
41 0.957829058170319
42 0.952003538608551
43 0.956550121307373
44 0.958868801593781
45 0.959625065326691
46 0.960244297981262
47 0.960377514362335
48 0.950835347175598
49 0.952841639518738
50 0.959105312824249
51 0.962208986282349
52 0.963455379009247
53 0.964364230632782
54 0.963271498680115
55 0.963827967643738
56 0.965114772319794
57 0.961261451244354
58 0.956338047981262
59 0.962351083755493
60 0.9652339220047
61 0.966645419597626
62 0.967311680316925
63 0.968519151210785
64 0.968912839889526
65 0.969216048717499
66 0.969650328159332
67 0.967077016830444
68 0.96728652715683
69 0.950484812259674
70 0.961421191692352
71 0.965921878814697
72 0.970019340515137
73 0.970864474773407
74 0.971773684024811
75 0.972114503383636
76 0.972982943058014
77 0.972904026508331
78 0.972892582416534
79 0.973300576210022
80 0.973526835441589
81 0.973495900630951
82 0.9730064868927
83 0.959217369556427
84 0.953817784786224
85 0.965136468410492
86 0.970264911651611
87 0.973215579986572
88 0.973960697650909
89 0.974767029285431
};
\addlegendentry{train}
\addplot [semithick, color1, mark=x, mark size=3, mark options={solid}]
table {%
9 0.791438937187195
19 0.87451434135437
29 0.897290349006653
39 0.902808725833893
49 0.909316182136536
59 0.908971190452576
69 0.907243490219116
79 0.91499799489975
89 0.917079091072083
};
\addlegendentry{test}
\end{axis}

\end{tikzpicture}

==> figures/unet.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,490); %set diagram left start at 0, and has height of 490

%Shape: Rectangle [id:dp36794488390759694] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (36,19) -- (83.97,19) -- (83.97,124.75) -- (36,124.75) -- cycle ;
%Shape: Rectangle [id:dp4617111431254024] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (110.35,124.75) -- (158.32,124.75) -- (158.32,230.5) -- (110.35,230.5) -- cycle ;
%Shape: Rectangle [id:dp5852561880899161] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (182.3,230.5) -- (230.27,230.5) -- (230.27,336.25) -- (182.3,336.25) -- cycle ;
%Shape: Rectangle [id:dp03959201730896855] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (254.25,336.25) -- (302.22,336.25) -- (302.22,442) -- (254.25,442) -- cycle ;
%Shape: Rectangle [id:dp17572137110566777] 
\draw   (566.03,19) -- (614,19) -- (614,124.75) -- (566.03,124.75) -- cycle ;
%Shape: Rectangle [id:dp6648384988882923] 
\draw   (494.08,124.75) -- (542.05,124.75) -- (542.05,230.5) -- (494.08,230.5) -- cycle ;
%Shape: Rectangle [id:dp5669900290245742] 
\draw   (422.13,230.5) -- (470.1,230.5) -- (470.1,336.25) -- (422.13,336.25) -- cycle ;
%Shape: Rectangle [id:dp7471777816891714] 
\draw   (350.18,336.25) -- (398.15,336.25) -- (398.15,442) -- (350.18,442) -- cycle ;
%Straight Lines [id:da568292586255944] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (103.15,69.76) -- (556.84,70.81) ;
\draw [shift={(558.84,70.82)}, rotate = 180.13] [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da6222159742905065] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (182.3,177.63) -- (472.9,178.68) ;
\draw [shift={(474.9,178.68)}, rotate = 180.21] [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da13378657961906848] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (254.25,283.38) -- (408.14,283.38) ;
\draw [shift={(410.14,283.38)}, rotate = 180] [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da43552624677490304] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (314.21,389.13) -- (338.59,389.13) ;
\draw [shift={(340.59,389.13)}, rotate = 180] [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;




\end{tikzpicture}

==> resnet.tex <==
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{axis}[
height=8cm,
legend cell align={left},
legend style={
  fill opacity=1,
  draw opacity=1,
  text opacity=1,
  at={(0.97,0.03)},
  anchor=south east,
  draw=white!80!black
},
tick align=outside,
tick pos=left,
width=10cm,
x grid style={white!69.0196078431373!black},
xlabel={Epoch},
xmajorgrids,
xmin=-0.5, xmax=208.5,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Dice Coef},
ymajorgrids,
ymin=0.479376070201397, ymax=0.840657688677311,
ytick style={color=black}
]
\addplot [semithick, color0, mark=x, mark size=3, mark options={solid}]
table {%
9 0.749181032180786
19 0.768976330757141
29 0.784484624862671
39 0.782566547393799
49 0.80383026599884
59 0.799732506275177
69 0.774044334888458
79 0.807013154029846
89 0.794789612293243
99 0.81143456697464
109 0.79976212978363
119 0.804109156131744
129 0.806172490119934
139 0.806680917739868
149 0.801862418651581
159 0.817336320877075
169 0.800456285476685
179 0.795554220676422
189 0.822798669338226
199 0.823730051517487
};
\addlegendentry{Segmentation}
\addplot [semithick, color1, mark=x, mark size=3, mark options={solid}]
table {%
9 0.511695384979248
19 0.545530736446381
29 0.579239189624786
39 0.617569208145142
49 0.650890827178955
59 0.665432929992676
69 0.710200548171997
79 0.730445086956024
89 0.755815982818604
99 0.776825368404388
109 0.78628808259964
119 0.7997887134552
129 0.790172696113586
139 0.803721129894257
149 0.817978501319885
159 0.813104033470154
169 0.821680963039398
179 0.824235796928406
189 0.820161938667297
199 0.824146747589111
};
\addlegendentry{Seg Random Decoder}
\addplot [semithick, color2, mark=x, mark size=3, mark options={solid}]
table {%
9 0.600777566432953
19 0.649967968463898
29 0.691806674003601
39 0.721601665019989
49 0.708280563354492
59 0.734398782253265
69 0.726153492927551
79 0.73738044500351
89 0.753463923931122
99 0.75335967540741
109 0.742675244808197
119 0.761210858821869
129 0.736369848251343
139 0.76499605178833
149 0.763383626937866
159 0.773019433021545
169 0.772840321063995
179 0.759884119033813
189 0.760068356990814
199 0.772546947002411
};
\addlegendentry{Classification}
\addplot [semithick, color3, mark=x, mark size=3, mark options={solid}]
table {%
9 0.495797961950302
19 0.512373745441437
29 0.589140892028809
39 0.581689596176147
49 0.654430687427521
59 0.635592639446259
69 0.625602602958679
79 0.642401397228241
89 0.657377481460571
99 0.674047231674194
109 0.678488612174988
119 0.692816972732544
129 0.693399786949158
139 0.670734405517578
149 0.700179278850555
159 0.705633878707886
169 0.700630903244019
179 0.691985130310059
189 0.698435664176941
199 0.700295686721802
};
\addlegendentry{Random}
\end{axis}

\end{tikzpicture}

